On the Use of Large Language Models to Generate Capability Ontologies

Capability ontologies are increasingly used to model functionalities of systems or machines. The creation of such ontological models with all properties and constraints of capabilities is very complex and can only be done by ontology experts. However, Large Language Models (LLMs) have shown that they can generate machine-interpretable models from natural language text input and thus support engineers / ontology experts. Therefore, this paper investigates how LLMs can be used to create capability ontologies. We present a study with a series of experiments in which capabilities with varying complexities are generated using different prompting techniques and with different LLMs. Errors in the generated ontologies are recorded and compared. To analyze the quality of the generated ontologies, a semi-automated approach based on RDF syntax checking, OWL reasoning, and SHACL constraints is used. The results of this study are very promising because even for complex capabilities, the generated ontologies are almost free of errors.

==> sections/Method.tex <==
% 1. Aufstellen der NL-TaskDescription. Inklusive aller Properties, Constraints usw.
% 2. Prompt wird automatisch generiert durch Befüllen eines Templates
% 3. Request an LLM, Ontologie liegt vor. dann Checks
% 4. Syntax-Validation. Wenn fail, dann Back-Prompt. Wenn dann immer noch fehlschlägt: Experte
% 5. Reasoning. Wenn fehlschlägt: Experte soll es sich anschauen mit den Explanations (eventuell Backprompting)
% 6. SHACL: Wenn Fehler: Backprompting
% (7. SPARQL, Competency Questions. Könnte aber auch in SHACL machen. Müssten durch user angelegt werden)
% 8. Check du Experten hinsichtlich Vollständigkeit
% Gesamt-Ergebnis: Enorme Arbeitserleichterung für Experten, aber kein einfach zu nutzender Automatismus
% 
This methodical study provides results that lead to a  proposal for the integration of an \gls{LLM} into a framework for the semi-automated generation of capability ontologies and addresses RQ 3. The \emph{LLM4Cap} framework is shown in Figure~\ref{fig:concept}. 

\begin{figure*}[htb]
    \centering
    \includegraphics[width=\linewidth]{figures/LLM4Cap.pdf}
    \caption{Overview of the proposed approach LLM4Cap for capability generation with \gls{LLM}. A natural language description of a capability is transformed via a \gls{LLM} to a capability ontology. The ontology is validated in four steps and backprompts found errors to the \gls{LLM} or forwarded to the expert.}
    \label{fig:concept}
\end{figure*}

The framework first requires a description of the capability to be generated in natural language as input.
It is important to describe all necessary elements or details of the capability, otherwise it cannot be modeled. 
The prompt is then generated automatically by replacing the task description in the meta prompt with the capability description. 
The meta prompt uses the few-shot prompting technique, as it has delivered the best results in the study.  
Overall, the prompt contains the already described elements: 
\begin{itemize}
    \item General instruction to translate the following task description describing a capability into an \gls{OWL} ontology in Turtle syntax based on the \gls{TBox} from the context description.  
    \item \gls{TBox} of the CaSk ontology to give context to the \gls{LLM} with possible classes and relations for the purpose of capability modeling.  
    \item Examples consisting of the capability description in natural language as input and the resulting capability ontology as output. The three examples from the study are used, applying the few-shot prompting technique. 
    \item Task description of the user's capability to create.
\end{itemize}  
The prompt is sent to Claude to generate the capability ontology, as this \gls{LLM} has shown better results in the study.
This is followed by a verification of the generated ontology. The verification takes place in three automated and one manual step:
First, the syntax check takes place, which was executed in the study with Protege, but can also be done automatically, e.g., in a script in Python with \emph{rdflib} or \emph{owlready2} library. Every character error and missing prefix is detected. 
The next step is to check the consistency of the ontology. The Pellet reasoner in Protege was used in the study to check for contradictions in the ontology. The owlready2 library, e.g., can be used for an automated check by integrating the \emph{Hermit} reasoner. For example, incorrect instances that belong to two disjoint classes are identified. 
For a more specific check of the ontology with regard to capabilities, further and more specific rules are used -- the developed \gls{SHACL} constraints from the study. This approach can identify hallucination of an \gls{LLM} -- information that is highly inaccurate or fabricated. Only relations defined in the \gls{SHACL} constraints are allowed to exist. Otherwise, invalid relations are detected and the ontology is inconsistent. In addition, these constraints provide initial indications of incompleteness by notifying if mandatory relations are missing. In the study, the \gls{SHACL} constraints were validated with Protege, while the \gls{SHACL} constraints could also be validated using the \emph{pyshacl} library in Python. 
All of these steps can be automated and reduce the effort required to create a capability ontology considerably. If errors are found in one of the three automated checks, the error is prompted back to the \gls{LLM}. \glspl{LLM} show good results in correcting errors with the inclusion of feedback \cite{Guan.2023}. The corrected result then goes through the same steps to verify the ontology. If the result repeatedly fails the same check, the result is passed to the expert. In the correction process, it can happen that an \gls{LLM} generates new errors which can lead to an endless loop. For this reason, the automated verification is then terminated. 
After a successful verification, the final step for the expert is to check the results. The final completeness can only be checked by the human expert who compares the generated ontology with the required capability elements. Many details of a capability cannot be checked automatically.   

% Hier eventuell noch die Anmerkung, dass Framework einer durchgehenden Anpassung / Entwicklung durchläuft? Gerade hinsichtlich Prompt Engineering. 


